HYperbolic Self-Paced Learning for Self-Supervised Skeleton-based Action Representations

Self-paced learning has been beneficial for tasks where some initial knowledge is available, such as weakly supervised learning and domain adaptation, to select and order the training sample sequence, from easy to complex. However its applicability remains unexplored in unsupervised learning, whereby the knowledge of the task matures during training. We propose a novel HYperbolic Self-Paced model (HYSP) for learning skeleton-based action representations. HYSP adopts self-supervision: it uses data augmentations to generate two views of the same sample, and it learns by matching one (named online) to the other (the target). We propose to use hyperbolic uncertainty to determine the algorithmic learning pace, under the assumption that less uncertain samples should be more strongly driving the training, with a larger weight and pace. Hyperbolic uncertainty is a by-product of the adopted hyperbolic neural networks, it matures during training and it comes with no extra cost, compared to the established Euclidean SSL framework counterparts. When tested on three established skeleton-based action recognition datasets, HYSP outperforms the state-of-the-art on PKU-MMD I, as well as on 2 out of 3 downstream tasks on NTU-60 and NTU-120. Additionally, HYSP only uses positive pairs and bypasses therefore the complex and computationally-demanding mining procedures required for the negatives in contrastive techniques. Code is available at https://github.com/paolomandica/HYSP.

==> fig/median_radius.tex <==
% \begin{figure*}[t] 
%     \centering
%     \subfloat[Pushing (Radius 0.9697)]{
%         \includegraphics[scale=0.10]{fig/images/medians/52_pushing_other_person_0_9697.pdf}
%         \label{fig:pushing}
%         }
%     \subfloat[Hugging (Radius 0.9672)]{
%         \includegraphics[scale=0.10]{fig/images/medians/55_hugging_other_person_0_9672.pdf}
%         \label{fig:hugging}
%         }
%     \subfloat[Walking apart (Radius 0.9692)]{
%         \includegraphics[scale=0.10]{fig/images/medians/60_walking_apart_from_each_other_0_9692.pdf}
%         \label{fig:walking_apart}
%         }
    
%     \bigskip
    
%     \subfloat[Take off hat (Radius 0.8143)]{
%         \includegraphics[scale=0.10]{fig/images/medians/21_take_off_a_hat_cap_0_8143.pdf}
%         \label{fig:take_off_hat}
%         }
%     \subfloat[Cheer up (Radius 0.8091)]{
%         \includegraphics[scale=0.10]{fig/images/medians/22_cheer_up_0_8091.pdf}
%         \label{fig:cheer_up}
%         }
%     \subfloat[Standing up (Radius 0.8538)]{
%         \includegraphics[scale=0.10]{fig/images/sequences/9_standing_up_from_sitting_position__0_8538.pdf}
%         \label{fig:standing_up}
%         }
%     % \subfloat[Reach into pocket (Radius 0.8193)]{
%     %     \includegraphics[scale=0.14]{fig/images/medians/25_reach_into_pocket_0_8193.pdf}
%     %     \label{fig:reach_pocket}
%     %     }
        
%     \bigskip
    
%     \subfloat[Playing with phone (Radius 0.7679)]{
%         \includegraphics[scale=0.10]{fig/images/medians/29_playing_with_phone_tablet_0_7679.pdf}
%         \label{fig:playing_phone}
%         }
%     % \subfloat[Typing on keyboard (Radius 0.7568)]{
%     %     \includegraphics[scale=0.14]{fig/images/medians/30_typing_on_a_keyboard_0_7568.pdf}
%     %     \label{fig:typing}
%     %     }
%     \subfloat[Writing (Radius 0.7721)]{
%         \includegraphics[scale=0.10]{fig/images/sequences/12_writing_0_7721.pdf}
%         \label{fig:writing}
%         }
%     \subfloat[Shake head (Radius 0.7181)]{
%         \includegraphics[scale=0.10]{fig/images/medians/36_shake_head_0_7181.pdf}
%         \label{fig:shake_head}
%         }
% \caption{Visualization of inter-class variability through skeleton sequences with high (a,b,c), average (d,e,f), and low (g,h,i) median radius.}
% \label{fig:inter_class_seq}
% \end{figure*}


\begin{figure*}[t] 
    \centering
    \subfloat[Writing (Radius 0.7712)]{
        \includegraphics[scale=0.11]{fig/images/sequences/12_writing_0_7712.pdf}
        \label{fig:writing}
        }
    \subfloat[Touch back (Radius 0.8108)]{
        \includegraphics[scale=0.11]{fig/images/sequences/46_touch_back_backache__0_8009.pdf}
        \label{fig:touch_back}
        }
    \subfloat[Standing up (Radius 0.8538)]{
        \includegraphics[scale=0.11]{fig/images/sequences/9_standing_up_from_sitting_position__0_8076.pdf}
        \label{fig:standing_up}
        }
\caption{Visualizations of skeleton samples. Uncertainty indicates the difficulty in classifying specific actions if they are characterized by less or more peculiar movements (a) and (b) or unambiguous actions (c).
}
\label{fig:skeleton_samples}
\end{figure*}

==> tex/Backup/2022-12-01_review_2_md.tex <==
# Reviewer 2

1. *I thank the authors for their detailed response to my concerns. I found the response to be adequate for the most part. Thanks for trying out the contrastive extension (6). I think that baseline should work but it can be explored as a part of future works. I agree with Reviewer GGZs, the general nature of this work should be explored in the future works as well.  
Given the batch size observation on the linear evaluation protocol, I am curious if it extends to other comparable skeleton-based SSL works. While not necessary, did the authors check this?  
I have increased my rating.*

----


1. Thank you for the appreciation and increment of rating. As suggested, we plan to investigate the general nature of hyperbolic self-paced learning on other SSL tasks.  
Regarding the batch size, we did not experiment with its effect on other methods. In fact, in Tables 1, 2, and 4, we report the performance of other SSL methods as provided by the original papers.  
Specifically, SkeletonCLR [1], CrossCLR [1] and AimCLR [2] use batch size of 128, P\&C [3], ISC [4] and MCC [5] set up the value at 64 and finally, 3s-Colorization [6], AS-CAL [7], $MS^2L$ [8] use 32. Given the different configurations, we have no reason to disbelieve that they did not optimize it yet. 

% Regarding the batch size, we have not tuned this parameter for other skeleton-based SSL works and reported the results directly from their papers. We plan to study this in detail in our future work. Thank you for the suggestion. \FG{Either state what in the alternative above, or just stop the answer after stating the no.}

---

[1] *3D Human Action Representation Learning via Cross-View Consistency Pursuit* (Li et al. CVPR 2021)  
[2] *Contrastive Learning from Extremely Augmented Skeleton Sequences for Self-supervised Action Recognition* (Guo et al. AAAI 2022)  
[3] *PREDICT & CLUSTER: Unsupervised Skeleton Based Action Recognition* (Su et al. CVPR 2020)  
[4] *Skeleton-Contrastive 3D Action Representation Learning* (Thoker et al. ACM Multimedia 2021)  
[5] *Self-supervised 3D Skeleton Action Representation Learning with Motion Consistency and Continuity* (Su et al. ICCV 2021)  
[6] *Skeleton cloud colorization for unsupervised 3D action representation learning* (Yang et al. ICCV 2021)  
[7] *Augmented skeleton based contrastive action learning with momentum LSTM for unsupervised action recognition* (Rao et al. Information Sciences 2021)  
[8] *MS2L: Multi-Task Self-Supervised Learning for Skeleton Based Action Recognition* (Lilang et al. ACMMM 2020)  




# Reviewer 3

1. *As in Table 3 and R4, the MoCo-only result is 69.7 on NTU 60 X-view. Is this the MoCo+hyperbolic result? As I know, the MoCo performance in [1] is 76.4 on NTU 60 X-view. Does this mean that HYSP reduces the performance of the MoCo-based method?*   

2. *I keep my mind that a better way to show the hyperbolic space is useful is to combine the hyperbolic space with multiple self-supervised learning baselines. As the authors mentioned, HYSP is designed for the negative-pair-free contrastive learning method. More experiments on this kind of method are needed.*  

3. *As shown in R3, the experimental results on NTU 60 increase when changing the batch size from 512 to 32. What about the NTU 120 dataset? For me, these two datasets are very similar, it is strange the comparison trend between HYSP and other methods on linear evaluation setting is different.*  

----

1. The reviewer correctly notes that the result "w/ negatives" in Table 3 represents MoCo in hyperbolic space, which is lower than the MoCo result of [1] in euclidean space. We explain this as the effect of using negatives in the hyperbolic SSL. Negatives help in euclidean SSL, since repulsing views from different samples reduces the chance of collapse. Repulsing in hyperbolic space also implies repulsing samples in terms of their value of uncertainty. We argue that this does not help, hence the lower performance of the hyperbolic MoCo. (Please also see Sec. 3.2.2, and our answer 6 to reviewer 2).
Note also that we experimented on adopting positive hyperbolic embeddings and negative euclidean ones (cf.\ \FG{answer X to reviewer X}, but this did not converge).
\LU{I don't think we have the results for this experiment. Should we remove this last sentence?}

% The is justified since MoCo also considers the comparison of negative pairs, pushing them apart. The repulsion of negatives makes sense in terms of angles (euclidean space) but not in terms of radius (certainty in hyperbolic space), hence their inclusion degrades the training in hyperbolic space.
% \FG{Put a reference to where discussed in the paper, and also in what points mentioned in our reply}

  

2. We tested HYSP on another negative-pair-free framework SimSiam [2]. Fortunately, the implementation is straightforward because the only differences with BYOL are in the target encoder not being updated with-momentum (same online and target encoders) and the addition of stop-gradient on the target branch to avoid collapsed representation. Then we experimented on NTU-60 xview with both euclidean SimSiam (66.3\% top-1 accuracy) and hyperbolic SimSiam (70.7\%). Our results demonstrate that the inclusion of hyperbolic pacing consistently improves the baseline SimSiam by 4.4\%. We will report the new results in the paper if allowed.  
Note that the adaption of HYSP to other self-supervised works is not straightforward and requires dedicated research.
For instance, Barlow Twins [3] changes the loss and needs a specific implementation correlation matrix for hyperbolic features. Similarly, SwAV [4] requires an appropriate hyperbolic clustering method which is an effort that ought separate work. 


3. We have not found any study on the sensitivity of the NTU-120 dataset to the variation of this specific hyper-parameter and therefore, we provide it here. The performance on NTU-120 remains consistent varying with the same values as the ablative study on NTU-60 (c.f. Table 5 in Appendix C), indeed changing the batch size from 16 to 512 results in fluctuations below 1\%. On the other hand, a significant change occurs only for extreme values, e.g., 61.5\% using batch size 8 (3.1\% drop) or 62.5\% using 1024 (2.1\% drop).


% 3. \FG{he asks why ntu120 experiments did not improve when testing for batch sizes, while NTU60 did. Hard to answer to his re-statement, without restating ourselves. Alternatives: (1) report literature where this is discussed; (2) report the actual numbers of NTU120 (so show that we did, but marginal changes); (3) take an apologetic/discursive approach: "As the reviewer notices, this result leaves us with the open question why the batch size does not affect in the case of the NTU120. In the absence of evidence, we refrain from statements, but agree that further research should shed light on this."} 

%\textbf{BM:I leave the below comment from Luca.}.
% Thank you for your comment. We agree that this result cannot be immediately explained and we . This is why we wrote in our reply to R2.1 that although we had tried to change the batch size on NTU-120 as well, the performance does not change and further research will certainly be done in the immediate future.  
% [1] *Vicreg: Variance-invariance-covariance regularization for self-supervised learning* (Bardes et al. ICLR 2022)  

---

[1] *3D Human Action Representation Learning via Cross-View Consistency Pursuit* (Li et al. CVPR 2021)  
[2] *Exploring Simple Siamese Representation Learning* (Chen et He, CVPR 2021)  
[3] *Barlow Twins: Self-Supervised Learning via Redundancy Reduction* (Zbontar et al. ICML 2021)  
[4] *Unsupervised Learning of Visual Features by Contrasting Cluster Assignments* (Caron et al. NeurIPS 2020)  


# Reviewer 4

1. *You mentioned that the “MoCo-only w/ neg.” is 69.7 while “MoCo-only” is 76.4 in CrosSCLR[1]. Since the method is only effective in the positive-only framework, it is hoped that its performance on methods such as SwAV[2] and SimSiam[3] can be verified in future work.*  
2. *You mentioned that “none of the most recent papers on skeleton-based SSL test image classification tasks”. I agree with this statement, but these methods all pay attention to the different characteristics of skeleton sequences compared to images. For example, the knowledge mining in CrossSCLR[1], spatio-temporal augmentations in AimCLR[4], motion consistency and motion continuity in MCC[5]. The method in this paper is more like a general improvement for BYOL, and does not fully consider the difference between images and skeleton sequences.*  

----


1. Thanks for your remark. We adopted self-paced learning with another positive-only framework SimSiam [1] and if permitted, we will report the new results in the paper.
Since the similarity of BYOL and SimSiam the implementation is straightforward, except for the addition of the stop-gradient to prevent collapse on the target branch and the adoption of same online and target encoder (removing momentum-update). Following that, we tested both euclidean and hyperbolic SimSiam on NTU-60 xview. The former results in 66.3\% and the latter in 70.7\% top-1 accuracy, showing hyperbolic pacing consistently improve the euclidean baseline (+4.4%).  
It is important to note that the adaptation of HYSP to other self-supervised works is not straightforward and requires a substantial research effort. For example, a specific implementation of a hyperbolic correlation matrix is required for Barlow Twins [2] when hyperbolic features are used. Likewise, SwAV [3] requires an appropriate hyperbolic clustering method which we leave for future work.

% 1. Thanks for your remark. We adopted self-paced learning with another positive-only framework SimSiam [1] and report results in Table X, Appendix X. The inclusion of HYSP brings consistent improvement in this SSL framework as well. Please see our response to R3.2, as well.

2. Thank you for your understanding. Actually, the amount of experiments to be reported for each case (skeleton-based or image classification) is generally so massive that all the papers considered are limited to one of the two cases. In fact, even the papers on SSL images do not report the skeleton's counterpart, although they are computationally more accessible. However, as rightly noted by the reviewer, HYSP can be considered a transversal and general SSL method, which will lead us to extend to the topic of images in future dedicated work.

---

[1] *Exploring Simple Siamese Representation Learning* (Chen et He CVPR 2021)  
[2] *Barlow Twins: Self-Supervised Learning via Redundancy Reduction* (Zbontar et al. ICML 2021)  
[3] *Unsupervised Learning of Visual Features by Contrasting Cluster Assignments* (Caron et al. NeurIPS 2020)   

==> tex/Backup/2022-12-01b_review-2.tex <==
# Reviewer 2

1. *I thank the authors for their detailed response to my concerns. I found the response to be adequate for the most part. Thanks for trying out the contrastive extension (6). I think that baseline should work but it can be explored as a part of future works. I agree with Reviewer GGZs, the general nature of this work should be explored in the future works as well.  
Given the batch size observation on the linear evaluation protocol, I am curious if it extends to other comparable skeleton-based SSL works. While not necessary, did the authors check this?  
I have increased my rating.*

----


1. Thank you for the appreciation and increment of rating. As suggested, we plan to investigate the general nature of HYSP on other SSL methods and tasks in the future.  
Regarding the batch size, we did not experiment on other methods. In fact, Tables 1, 2, and 4 report the performances from the original papers. However, we have found several notes on batch sizes in literature: SkeletonCLR [1], CrossCLR [1] and AimCLR [2] use a batch size of 128; P\&C [3], ISC [4] and MCC [5] use 64; 3s-Colorization [6], AS-CAL [7], and $MS^2L$ [8] use 32. So we have no reason to believe that they disregarded this hyperparameter. 

% Regarding the batch size, we have not tuned this parameter for other skeleton-based SSL works and reported the results directly from their papers. We plan to study this in detail in our future work. Thank you for the suggestion. \FG{Either state what in the alternative above, or just stop the answer after stating the no.}

---

[1] *3D Human Action Representation Learning via Cross-View Consistency Pursuit* (Li et al. CVPR 2021)  
[2] *Contrastive Learning from Extremely Augmented Skeleton Sequences for Self-supervised Action Recognition* (Guo et al. AAAI 2022)  
[3] *PREDICT & CLUSTER: Unsupervised Skeleton Based Action Recognition* (Su et al. CVPR 2020)  
[4] *Skeleton-Contrastive 3D Action Representation Learning* (Thoker et al. ACM Multimedia 2021)  
[5] *Self-supervised 3D Skeleton Action Representation Learning with Motion Consistency and Continuity* (Su et al. ICCV 2021)  
[6] *Skeleton cloud colorization for unsupervised 3D action representation learning* (Yang et al. ICCV 2021)  
[7] *Augmented skeleton based contrastive action learning with momentum LSTM for unsupervised action recognition* (Rao et al. Information Sciences 2021)  
[8] *MS2L: Multi-Task Self-Supervised Learning for Skeleton Based Action Recognition* (Lilang et al. ACMMM 2020)  




# Reviewer 3

1. *As in Table 3 and R4, the MoCo-only result is 69.7 on NTU 60 X-view. Is this the MoCo+hyperbolic result? As I know, the MoCo performance in [1] is 76.4 on NTU 60 X-view. Does this mean that HYSP reduces the performance of the MoCo-based method?*   

2. *I keep my mind that a better way to show the hyperbolic space is useful is to combine the hyperbolic space with multiple self-supervised learning baselines. As the authors mentioned, HYSP is designed for the negative-pair-free contrastive learning method. More experiments on this kind of method are needed.*  

3. *As shown in R3, the experimental results on NTU 60 increase when changing the batch size from 512 to 32. What about the NTU 120 dataset? For me, these two datasets are very similar, it is strange the comparison trend between HYSP and other methods on linear evaluation setting is different.*  

----

1. The reviewer correctly notes that the result "w/ negatives" in Table 3 represents MoCo in hyperbolic space, which is lower than the MoCo result of [1] in Euclidean space. We explain this as the effect of using negatives in the hyperbolic SSL. Negatives help in the Euclidean SSL, since repulsing views from different samples reduces the chance of collapse. Repulsing in hyperbolic space also implies repulsing samples in terms of their value of uncertainty. We argue that this does not help, hence the lower performance of the hyperbolic MoCo. (Please also see Sec. 3.2.2, and our answer 6 to reviewer 2).
Note also that we experimented on adopting positive hyperbolic embeddings and negative Euclidean ones (cf.\ answer 6 to reviewer 2, but this did not converge).
%\LU{I don't think we have the results for this experiment. Should we remove this last sentence?}\FG{I referred to R2.6, where you test the hybrid. But it seems you refer to R2.6 here for our note on the need of positives only, which was probably a different answer?}

% The is justified since MoCo also considers the comparison of negative pairs, pushing them apart. The repulsion of negatives makes sense in terms of angles (Euclidean space) but not in terms of radius (certainty in hyperbolic space), hence their inclusion degrades the training in hyperbolic space.
% \FG{Put a reference to where discussed in the paper, and also in what points mentioned in our reply}

  

2. Your observation has been a stimulus to test HYSP on a second positive-only SSL method: SimSiam [2].  On the NTU-60 xview, the Euclidean SimSiam yields 66.3\% top-1 accuracy, which is lower than the Euclidean BYOL (82.6\%, see Table 1), consistently with the literature. The HYSP variant of SimSiam yields 70.7\%. So HYSP improves also in this case.  
Let us note that adapting HYSP to other SSL methods is not straightforward. For instance, Barlow Twins [3] adopts a different loss and requires a correlation matrix of hyperbolic features. Similarly, SwAV [4] requires to cluster features in the hyperbolic space. We argue that further dedicated research is required in those cases.

%Fortunately, the implementation is straightforward because the only differences with BYOL are in the target encoder not being updated with-momentum (same online and target encoders) and the addition of stop-gradient on the target branch to avoid collapsed representation. Then we experimented on NTU-60 xview with both Euclidean SimSiam (66.3\% top-1 accuracy) and hyperbolic SimSiam (70.7\%). Our results demonstrate that the inclusion of hyperbolic pacing consistently improves the baseline SimSiam by 4.4\%. We will report the new results in the paper if allowed.  



5. We have not found references to the sensitivity of SSL methods to batch size variations on the NTU120 dataset in the literature, so we have performed further experiments. When changing the batch size from 16 to 512, the performance of HYSP on the NTU120 xset only changes by 1\%. Significant changes can only be observed outside this range, e.g., 61.5\% top-1 accuracy xset with a batch size 8 (3.1\% performance drop), 62.5\% with 1024 (2.1\% drop). This robustness is good news, but it does not address why the NTU-120 linear protocol is the sole where HYSP does not outperform the state-of-the-art. As noted in answer 1 to reviewer 2, this remains to be addressed in future research.


% 3. \FG{he asks why ntu120 experiments did not improve when testing for batch sizes, while NTU60 did. Hard to answer to his re-statement, without restating ourselves. Alternatives: (1) report literature where this is discussed; (2) report the actual numbers of NTU120 (so show that we did, but marginal changes); (3) take an apologetic/discursive approach: "As the reviewer notices, this result leaves us with the open question why the batch size does not affect in the case of the NTU120. In the absence of evidence, we refrain from statements, but agree that further research should shed light on this."} 

%\textbf{BM:I leave the below comment from Luca.}.
% Thank you for your comment. We agree that this result cannot be immediately explained and we . This is why we wrote in our reply to R2.1 that although we had tried to change the batch size on NTU-120 as well, the performance does not change and further research will certainly be done in the immediate future.  
% [1] *Vicreg: Variance-invariance-covariance regularization for self-supervised learning* (Bardes et al. ICLR 2022)  

---

[1] *3D Human Action Representation Learning via Cross-View Consistency Pursuit* (Li et al. CVPR 2021)  
[2] *Exploring Simple Siamese Representation Learning* (Chen et He, CVPR 2021)  
[3] *Barlow Twins: Self-Supervised Learning via Redundancy Reduction* (Zbontar et al. ICML 2021)  
[4] *Unsupervised Learning of Visual Features by Contrasting Cluster Assignments* (Caron et al. NeurIPS 2020)  


# Reviewer 4

1. *You mentioned that the “MoCo-only w/ neg.” is 69.7 while “MoCo-only” is 76.4 in CrosSCLR[1]. Since the method is only effective in the positive-only framework, it is hoped that its performance on methods such as SwAV[2] and SimSiam[3] can be verified in future work.*  
2. *You mentioned that “none of the most recent papers on skeleton-based SSL test image classification tasks”. I agree with this statement, but these methods all pay attention to the different characteristics of skeleton sequences compared to images. For example, the knowledge mining in CrossSCLR[1], spatio-temporal augmentations in AimCLR[4], motion consistency and motion continuity in MCC[5]. The method in this paper is more like a general improvement for BYOL, and does not fully consider the difference between images and skeleton sequences.*  

----


1. Thanks for your remark. We adopted self-paced learning with another positive-only framework SimSiam [1] and if permitted, we will report the new results in the paper.
Since the similarity of BYOL and SimSiam the implementation is straightforward, except for the addition of the stop-gradient to prevent collapse on the target branch and the adoption of same online and target encoder (removing momentum-update). Following that, we tested both Euclidean and hyperbolic SimSiam on NTU-60 xview. The former results in 66.3\% and the latter in 70.7\% top-1 accuracy, showing hyperbolic pacing consistently improve the Euclidean baseline (+4.4\%).  
It is important to note that the adaptation of HYSP to other self-supervised works is not straightforward and requires a substantial research effort. For example, a specific implementation of a hyperbolic correlation matrix is required for Barlow Twins [2] when hyperbolic features are used. Likewise, SwAV [3] requires an appropriate hyperbolic clustering method which we leave for future work.

% 1. Thanks for your remark. We adopted self-paced learning with another positive-only framework SimSiam [1] and report results in Table X, Appendix X. The inclusion of HYSP brings consistent improvement in this SSL framework as well. Please see our response to R3.2, as well.

2. Thank you for your understanding. Actually, the amount of experiments to be reported for each case (skeleton-based or image classification) is generally so massive that all the papers considered are limited to one of the two cases. In fact, even the papers on SSL images do not report the skeleton's counterpart, although they are computationally more accessible. However, as rightly noted by the reviewer, HYSP can be considered a transversal and general SSL method, which will lead us to extend to the topic of images in future dedicated work.

---

[1] *Exploring Simple Siamese Representation Learning* (Chen et He CVPR 2021)  
[2] *Barlow Twins: Self-Supervised Learning via Redundancy Reduction* (Zbontar et al. ICML 2021)  
[3] *Unsupervised Learning of Visual Features by Contrasting Cluster Assignments* (Caron et al. NeurIPS 2020)   

==> tex/Backup/2022-12-02_rev_2_bk.tex <==
# Reviewer 2

1. *I thank the authors for their detailed response to my concerns. I found the response to be adequate for the most part. Thanks for trying out the contrastive extension (6). I think that baseline should work but it can be explored as a part of future works. I agree with Reviewer GGZs, the general nature of this work should be explored in the future works as well.  
Given the batch size observation on the linear evaluation protocol, I am curious if it extends to other comparable skeleton-based SSL works. While not necessary, did the authors check this?  
I have increased my rating.*

----


1. Thank you for the appreciation and increment of rating. As suggested, we plan to investigate the general nature of HYSP on other SSL methods and tasks in the future.  
Regarding the batch size, we did not experiment on other methods. In fact, Tables 1, 2, and 4 report the performances from the original papers. However, we have found several notes on batch sizes in literature: SkeletonCLR [1], CrossCLR [1] and AimCLR [2] use a batch size of 128; P\&C [3], ISC [4] and MCC [5] use 64; 3s-Colorization [6], AS-CAL [7], and $MS^2L$ [8] use 32. So we have no reason to believe that they disregarded tuning this hyperparameter. 

% Regarding the batch size, we have not tuned this parameter for other skeleton-based SSL works and reported the results directly from their papers. We plan to study this in detail in our future work. Thank you for the suggestion. \FG{Either state what in the alternative above, or just stop the answer after stating the no.}

---

[1] *3D Human Action Representation Learning via Cross-View Consistency Pursuit* (Li et al. CVPR 2021)  
[2] *Contrastive Learning from Extremely Augmented Skeleton Sequences for Self-supervised Action Recognition* (Guo et al. AAAI 2022)  
[3] *PREDICT & CLUSTER: Unsupervised Skeleton Based Action Recognition* (Su et al. CVPR 2020)  
[4] *Skeleton-Contrastive 3D Action Representation Learning* (Thoker et al. ACM Multimedia 2021)  
[5] *Self-supervised 3D Skeleton Action Representation Learning with Motion Consistency and Continuity* (Su et al. ICCV 2021)  
[6] *Skeleton cloud colorization for unsupervised 3D action representation learning* (Yang et al. ICCV 2021)  
[7] *Augmented skeleton based contrastive action learning with momentum LSTM for unsupervised action recognition* (Rao et al. Information Sciences 2021)  
[8] *MS2L: Multi-Task Self-Supervised Learning for Skeleton Based Action Recognition* (Lilang et al. ACMMM 2020)  




# Reviewer 3

1. *As in Table 3 and R4, the MoCo-only result is 69.7 on NTU 60 X-view. Is this the MoCo+hyperbolic result? As I know, the MoCo performance in [1] is 76.4 on NTU 60 X-view. Does this mean that HYSP reduces the performance of the MoCo-based method?*   

2. *I keep my mind that a better way to show the hyperbolic space is useful is to combine the hyperbolic space with multiple self-supervised learning baselines. As the authors mentioned, HYSP is designed for the negative-pair-free contrastive learning method. More experiments on this kind of method are needed.*  

3. *As shown in R3, the experimental results on NTU 60 increase when changing the batch size from 512 to 32. What about the NTU 120 dataset? For me, these two datasets are very similar, it is strange the comparison trend between HYSP and other methods on linear evaluation setting is different.*  

----

1. The reviewer correctly notes that the result "w/ negatives" in Table 3 represents MoCo in hyperbolic space, which is lower than the MoCo result of [1] in Euclidean space. We explain this as the effect of using negatives in the hyperbolic SSL. Negatives help in the Euclidean SSL, since repulsing views from different samples reduces the chance of collapse. Repulsing in hyperbolic space also implies repulsing samples in terms of their value of uncertainty. We argue that this does not help, hence the lower performance of the hyperbolic MoCo. (Please also see Sec. 3.2.2, and our answer 6 to reviewer 2).
Note also that we experimented on adopting positive hyperbolic embeddings and negative Euclidean ones (cf.\ answer 6 to reviewer 2, but this did not converge).
%\LU{I don't think we have the results for this experiment. Should we remove this last sentence?}\FG{I referred to R2.6, where you test the hybrid. But it seems you refer to R2.6 here for our note on the need of positives only, which was probably a different answer?}

% The is justified since MoCo also considers the comparison of negative pairs, pushing them apart. The repulsion of negatives makes sense in terms of angles (Euclidean space) but not in terms of radius (certainty in hyperbolic space), hence their inclusion degrades the training in hyperbolic space.
% \FG{Put a reference to where discussed in the paper, and also in what points mentioned in our reply}

  

2. Your observation has been a stimulus to test HYSP on a second positive-only SSL method: SimSiam [2].  On the NTU-60 *xview*, the Euclidean SimSiam yields 66.3\% top-1 accuracy, which is lower than the Euclidean BYOL (82.6\%, see Table 1), consistently with the literature. The HYSP variant of SimSiam yields 70.7\%. So HYSP improves also in this case.  
Let us note that adapting HYSP to other SSL methods is not straightforward. For instance, Barlow Twins [3] adopts a different loss, and a hyperbolic variant may require a correlation matrix of hyperbolic features. Similarly, a hyperbolic variant of SwAV [4] may require clustering features in the hyperbolic space. We argue that further dedicated research is needed in those cases.

%Fortunately, the implementation is straightforward because the only differences with BYOL are in the target encoder not being updated with-momentum (same online and target encoders) and the addition of stop-gradient on the target branch to avoid collapsed representation. Then we experimented on NTU-60 *xview* with both Euclidean SimSiam (66.3\% top-1 accuracy) and hyperbolic SimSiam (70.7\%). Our results demonstrate that the inclusion of hyperbolic pacing consistently improves the baseline SimSiam by 4.4\%. We will report the new results in the paper if allowed.  



5. We have not found references to the sensitivity of SSL methods to batch size variations on the NTU120 dataset in the literature, so we have performed further experiments. When changing the batch size from 16 to 512, the performance of HYSP on the NTU120 _xset_ only changes by 1\%. Significant changes can only be observed outside this range, e.g., 61.5\% top-1 accuracy *xset* with a batch size 8 (3.1\% performance drop), 62.5\% with 1024 (2.1\% drop). This robustness is good news, but it does not address why the NTU-120 linear protocol is the sole where HYSP does not outperform the state-of-the-art. As noted in answer 1 to reviewer 2, this remains to be addressed in future research.


% 3. \FG{he asks why ntu120 experiments did not improve when testing for batch sizes, while NTU60 did. Hard to answer to his re-statement, without restating ourselves. Alternatives: (1) report literature where this is discussed; (2) report the actual numbers of NTU120 (so show that we did, but marginal changes); (3) take an apologetic/discursive approach: "As the reviewer notices, this result leaves us with the open question why the batch size does not affect in the case of the NTU120. In the absence of evidence, we refrain from statements, but agree that further research should shed light on this."} 

%\textbf{BM:I leave the below comment from Luca.}.
% Thank you for your comment. We agree that this result cannot be immediately explained and we . This is why we wrote in our reply to R2.1 that although we had tried to change the batch size on NTU-120 as well, the performance does not change and further research will certainly be done in the immediate future.  
% [1] *Vicreg: Variance-invariance-covariance regularization for self-supervised learning* (Bardes et al. ICLR 2022)  

---

[1] *3D Human Action Representation Learning via Cross-View Consistency Pursuit* (Li et al. CVPR 2021)  
[2] *Exploring Simple Siamese Representation Learning* (Chen et He, CVPR 2021)  
[3] *Barlow Twins: Self-Supervised Learning via Redundancy Reduction* (Zbontar et al. ICML 2021)  
[4] *Unsupervised Learning of Visual Features by Contrasting Cluster Assignments* (Caron et al. NeurIPS 2020)  


# Reviewer 4

1. *You mentioned that the “MoCo-only w/ neg.” is 69.7 while “MoCo-only” is 76.4 in CrosSCLR[1]. Since the method is only effective in the positive-only framework, it is hoped that its performance on methods such as SwAV[2] and SimSiam[3] can be verified in future work.*  
2. *You mentioned that “none of the most recent papers on skeleton-based SSL test image classification tasks”. I agree with this statement, but these methods all pay attention to the different characteristics of skeleton sequences compared to images. For example, the knowledge mining in CrossSCLR[1], spatio-temporal augmentations in AimCLR[4], motion consistency and motion continuity in MCC[5]. The method in this paper is more like a general improvement for BYOL, and does not fully consider the difference between images and skeleton sequences.*  

----


1. Thanks for your remark. In this time, allotted for discussion, we have implemented a HYSP variant of the positive-only SimSiam [1] and verified a performance improvement when turning from Euclidean to hyperbolic self-pacing, \FG{"comparable"? is this in the same order of magnitude? else remove what follows} \PL{The absolute values are lower but the increment is comparable. With BYOL the difference is 5.7\%.} \LU{I agree with Paolo. Do we want to add a sentence as the one in 3.2: "which is lower than the Euclidean BYOL (82.6\%, see Table 1), consistently with the literature"} to the case of BYOL. On NTU-60 *xview*, the Euclidean SimSiam yields 66.3\% top-1 accuracy, while the HYSP variant of SimSiam scores 70.7\%, improving by +4.4\%. We confirm that the further adaptation of HYSP to other SSL methods requires dedicated research efforts. For example, a hyperbolic correlation matrix may be required for Barlow Twins [2], and the adoption of hyperbolic clustering may be required for SwAV [3].

%\FG{check the way that we write xview and xset across all instances and adopt a consistent font style, be that italic, with "quotes", or just plain}. 

%Since the similarity of BYOL and SimSiam the implementation is straightforward, except for the addition of the stop-gradient to prevent collapse on the target branch and the adoption of same online and target encoder (removing momentum-update). Following that, we tested both Euclidean and hyperbolic SimSiam 


% 1. Thanks for your remark. We adopted self-paced learning with another positive-only framework SimSiam [1] and report results in Table X, Appendix X. The inclusion of HYSP brings consistent improvement in this SSL framework as well. Please see our response to R3.2, as well.

2. Thanks for your understanding and for re-stating the generality of the HYSP proposition across skeleton-based action and image representations, which we appreciate. We will treasure this consideration in future work. \FG{I'm not really feeling willing to push further against this reviewer. Our point 1 on SimSiam is very strong. The reviewer understood very well, but she/he pushes back, and further insisting will not help. Let us see what he says about point 1.} \LU{That's ok, we agree with that!}

%Please consider that the times for training and cross-validating hyper-parameters are conspicuous.
%Thank you for your understanding. Actually, the amount of experiments to be reported for each case (skeleton-based or image classification) is generally so massive that all the papers considered are limited to one of the two cases. In fact, even the papers on SSL images do not report the skeleton's counterpart, although they are computationally more accessible. However, as rightly noted by the reviewer, HYSP can be considered a transversal and general SSL method, which will lead us to extend to the topic of images in future dedicated work.

---

[1] *Exploring Simple Siamese Representation Learning* (Chen et He CVPR 2021)  
[2] *Barlow Twins: Self-Supervised Learning via Redundancy Reduction* (Zbontar et al. ICML 2021)  
[3] *Unsupervised Learning of Visual Features by Contrasting Cluster Assignments* (Caron et al. NeurIPS 2020)   

==> tex/Backup/rev_bk_2022-11-15.tex <==
%\vspace{-14cm}
\noindent We are thankful to the reviewers for their appreciation and detailed suggestions. In the following discussion points, \textbf{R\textit{x}.\textit{y}} denotes point \textit{y} from reviewer \textit{x}. All changes in the resubmitted manuscript are in \CH{red}, for easier readability.\\


\noindent \textbf{Reviewer 1}\\

\noindent \textbf{R1.1} \textit{While I did not find any major concerns with the work, I am curious how the choice and the quality of positive samples affect performance. For example, how much does the performance depend on "hard positives"? Fig. 3a shows the correlation between the feature distances and the uncertainties. If only samples corresponding to the last few columns were to be used in the training (which I'm assuming are the hardest samples), how much would the performance drop? Since humans can perform similar actions with many diverse movements, real-world data can contain many such hard positives.}\\
\indent ANSWER \\

%\noindent \textbf{R1.2} \textit{In addition to showing the inter-class variability (Sec. 4.4 and appendix), it can be illuminating to also see the confusion matrix, showing how the variability might be correlated with the per-class performance.}\\
\noindent \textbf{R1.2} \textit{Regarding the confusion matrix and correlation of variability.} \LU{We changed the question?}\\
%We are thankful for the suggestion,
\indent We thanks the reviewer for this suggestion. We have produced the confusion matrix and show it in Fig. \ref{fig:confmat}.  The result leads to some interesting insights. 
The classes are sorted by the median radius per action class in descending order (See also Fig. 4 in Appendix A). Top-1 accuracy and uncertainty are correlated; indeed, we have high values in the diagonal for the top-left part (class with higher certainty), resulting in lower misclassification (and variability) with other classes. On the other hand, for the bottom-right part (classes with lower certainty), we have lower values on the diagonal and predictions are spread in similar classes, resulting in higher variability. For easier readability, we report following list of correspondence between class ID and the relative action.

% The model performs accurate predictions for almost all the classes (high values in the diagonal). There are just with few exceptions due to actions with small and ambiguous movements. In example the action \textit{Clapping} (number 9) is confused with \textit{Rub two hands together} (number 33), \textit{Writing} (number 11) is confused with \textit{Playing with phone/tablet} (number 28) or \textit{Typing on a keyboard} (number 30). Or misclassification is due to very similar actions: in examples \textit{Wear a shoe} (number 15) is confused with \textit{Take off a shoe} (number 16). 

% There are also other minor inaccuracies, that are all very plausible, like: \textit{Wipe face} (number 36) is confused with \textit{Brushing hair} (number 4) or \textit{Sneeze/cough} (number 40) is confused with \textit{Touch head (headache) (number 43) and Nausea/Vomiting condition} (number 47).

\noindent We add this study to the supplementary material (See Appendix A) so that it is available to all. \LU{Update supp mat}

\FG{He asked for a comment on correlation of variability (as we state it in appendix A) and the per-class performance, while the current answer seems a bit more generic. What do you think? Eg you might sort the confusion matrix entries according to Fig 4. Then you might better comment on the errors, and the correlations (whether errors are positioned higher in the tables).} \LU{Changed as we discussed, please double check the comment part and caption}
\\

\newpage
\begin{figure*}[h] 
\centering
\includegraphics[width=\columnwidth]{fig/rebuttal/confmat_top1_acc=82.6.pdf}
\caption{Confusion matrix for NTU60 \textit{xview} with single stream input. The evaluation protocol adopted is the \textit{linear}. The classes are sorted by the median radius per action class in descending order (See also Fig. 4 in Appendix A). Top-1 accuracy and uncertainty are correlated indeed, we have high values in the diagonal for the top-left part (High certainty per class) and higher variability in classification for the bottom-right part (Low certainty per class).
For easier readability, we report following list of correspondence between class ID and the relative action.}
% For almost all classes (high diagonal values), the model performs well. Exceptions are actions with small and ambiguous movements like: \textit{Clapping} (number 9) is confused with \textit{Rub two hands together} (number 33) or misclassification caused by similar actions like: \textit{Wear a shoe} (number 15) is confused with \textit{Take off a shoe} (number 16). For easier readability, we report following list of correspondence between class ID and the relative action.}

\label{fig:confmat}
\end{figure*}

\begin{multicols}{4}
    \tiny
    \begin{itemize}
    \setlength\itemsep{0.1em}
        \item 0. drink water.
        \item 1. eat meal/snack.
        \item 2. brushing teeth.
        \item 3. brushing hair.
        \item 4. drop.
        \item 5. pickup.
        \item 6. throw.
        \item 7. sitting down.
        \item 8. standing up (from sitting position).
        \item 9. clapping.
        \item 10. reading.
        \item 11. writing.
        \item 12. tear up paper.
        \item 13. wear jacket.
        \item 14. take off jacket.
        \item 15. wear a shoe.
        \item 16. take off a shoe.
        \item 17. wear on glasses.
        \item 18. take off glasses.
        \item 19. put on a hat/cap.
        \item 20. take off a hat/cap.
        \item 21. cheer up.
        \item 22. hand waving.
        \item 23. kicking something.
        \item 24. reach into pocket.
        \item 25. hopping (one foot jumping).
        \item 26. jump up.
        \item 27. make a phone call/answer phone.
        \item 28. playing with phone/tablet.
        \item 29. typing on a keyboard.
        \item 30. pointing to something with finger.
        \item 31. taking a selfie.
        \item 32. check time (from watch).
        \item 33. rub two hands together.
        \item 34. nod head/bow.
        \item 35. shake head.
        \item 36. wipe face.
        \item 37. salute.
        \item 38. put the palms together.
        \item 39. cross hands in front (say stop).
        \item 30. sneeze/cough.
        \item 41. staggering.
        \item 42. falling.
        \item 43. touch head (headache).
        \item 44. touch chest (stomachache/heart pain).
        \item 45. touch back (backache).
        \item 46. touch neck (neckache).
        \item 47. nausea or vomiting condition.
        \item 48. use a fan (with hand or paper)/feeling warm.
        \item 49. punching/slapping other person.
        \item 50. kicking other person.
        \item 51. pushing other person.
        \item 52. pat on back of other person.
        \item 53. point finger at the other person.
        \item 54. hugging other person.
        \item 55. giving something to other person.
        \item 56. touch other person's pocket.
        \item 57. handshaking.
        \item 58. walking towards each other.
        \item 59. walking apart from each other.
    \end{itemize}
\end{multicols}




\noindent \textbf{Reviewer 2}\\


% \begin{table*}
% \caption{Top-1 accuracy varying batch size for the linear protocol. The dataset used in this table is NTU-60 xview.}
% \centering
% \resizebox{0.3\textwidth}{!}{%
% \begin{tabular}{c|c}
% \toprule
% Batch size & Top-1 Acc.\\
% \midrule
% 512 & 78.3 \\
% 256 & 79.9 \\
% 128 & 81.2 \\
% 64 & 82.2 \\
% \textbf{32} & \textbf{82.6} \\
% \bottomrule
% \end{tabular}
% }
% \label{tab:bs_linear}
% \end{table*}


\begin{table*}
\caption{Top-1 accuracy varying batch size for the linear protocol. The dataset used in this table is NTU-60 xview.}
\centering
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{r|ccccc}
\toprule
Batch size & 512 & 256 & 128 & 64 & \textbf{32}\\
\midrule
Top-1 Acc. & 78.3 & 79.9 & 81.2 & 82.2 & \textbf{82.6}\\
\bottomrule
\end{tabular}
}
\label{tab:bs_linear}
\end{table*}



\noindent \textbf{R2.1} \textit{While the approach shows good improvements on semi-supervised learning, these do not hold for the other settings. The comparison for finetuning would have been easier if there were numbers reported for ISC.}\\
\indent Thank you for the appropriate comment. Unfortunately, the \FG{from here} finetuning results for \citet{thoker2021skeleton} are not available on their paper \FG{to here, is enough} and we do not have the resources to train it from scratch at the moment \FG{no need for an apology}. We think that by outperforming it with a good gap using a fraction of the label (10\% in the semi-supervised protocol), it is reasonable to think that HYSP can perform better than or equal to ISC using all the labels (finetuning protocol).
\FG{Not sure that it is reasonable to say that we outperform it, given the semi-sup experiments. It'd be more sensible to speak about the large margin improvement of our technique wrt ISP.}

\indent \PL{Thank you for the appropriate comment. Unfortunately, the finetuning results for \citet{thoker2021skeleton} are not available on their paper. However, looking at the ranking of our method in other protocols and datasets, it is reasonable to think that we should perform better or equal than ISC even in the finetuning one.}

Thanks to your comment and \textbf{R3.3}, we re-checked the results obtained with the linear protocol and we were able to improve \FG{not recommendable to speak about improvement wrt our submission. Our paper will only be judged according to what we submitted} the results significantly up to the state-of-the-art on NTU-60 and PKUMMD I with this protocol. \FG{previous text in the paragraph not needed, starting answer from here seems ok}

\PL{As a result of your comments, we investigated the reasons why HYSP did not achieve the expected performance on the linear protocol as it did on the other protocols. We discovered that this particular protocol benefits, especially on NTU-60, from a batch size much lower than usual. For example, using batch size 32 (as opposed to the previous value of 512) the accuracy goes from 78.3 to 82.6 (+4.3\%) on the xview subset. For a complete analysis, we have added Table \ref{tab:bs_linear} where you can see the increase in top-1 accuracy as the batch size changes.}

We, therefore, rdid all experiments where the linear protocol was adopted that shifted all the results uniformly. Particularly look at Tables 1 and 3, where we marked all the changes in red. 
Both for NTU-60 (both xsub and xview) and PKUMMD I we have a significant increase of the performance in the single-stream case and consistently in the 3-stream case leading to the achievement of the state-of-the-art. However, it is interesting that for NTU-120 varying the batch size does not lead to any change in performance. Thus, while for NTU-60 and PKUMMD I we found this interesting property thanks to your comment, and will report on it in the supplementary material (See Appendix C) together with the full collection of all model checkpoints for complete transparency \LU{FOOTNOTE Link}, the case of NTU-120 remains open for further investigation, which we will address in the near future. \PL{I think we can substitute all of this with a single sencence (see below).}

\PL{Therefore, we re-evaluated the model on the linear protocol with batch-size 32 and we updated the results where needed (Tables 1 and 3).}

Please check also answer to \textbf{R2.7} about the Transfer Learning protocol.
\\


\noindent \textbf{R2.2} \textit{It is not clear from the paper why hyperbolic specifically. The Section 3.2, directly starts with explaining how a hyperbolic extension to SkeletonCLR would work. As far as I understand, the hyperbolic geometry is useful to encode hierarchies, tree-like structures. It is not clear to me why the problem being tackled by this paper needs that.}\\
\indent Thanks for the remark. We added a clarification on the meaning of uncertainty in the specific case of human motion for action classification, thanks also to the comment \textbf{R2.3}.

\LU{Maybe I would change a few sentences on the use of hyperbolic geometry in the introduction}. 
The hyperbolic geometry gives, as a free by-product, the uncertainty of each sample (defined as $1 -$ radius). Our intuition for the paper comes from the fact that this extra radius knowledge can add information to the self-supervision signal for the pretext task. 
If we reason in polar coordinates, each sample can be decomposed in a radius and an angle. SkeletonCLR being in Euclidean space matches the positive sample by reducing only the angle distance with the relative reference sample. In this way, the radius is not taken into account, which is not the case using hyperbolic space and, thus, HYSP.

If we consider all the samples of a specific class, the hierarchy that is derived is structured on the variety of movements that can be made to perform the same action. At the top of the hierarchy (samples with low radius and high uncertainty) we find small and uncharacteristic movements for that action. Descending gradually toward the base of the hierarchy (samples with high radius and low uncertainty), we have movements that are more peculiar and very wide. 
Thus a hyperbolic model is able to structure and encode the complex intra-class relationships (as well as inter-class ones) to obtain better representations over each evaluation protocol.

\PL{The hyperbolic geometry gives, as a free by-product, the uncertainty of each sample (defined as $1 -$ radius). Our intuition is that this extra radius knowledge can add information to the self-supervision signal for the pretext task. 
Reasoning in polar coordinates, each representation is characterized by a radius and an angle. In both Euclidean (e.g. SkeletonCLR) and Hyperbolic space the goal is to minimize the angle between positive samples. The difference lies in the fact that in Hyperbolic space we can also leverage the radius to self-pace the learning process, which is not possible in the Euclidean case. A Hyperbolic model is, therefore, able to encode and exploit the complex intra- and inter-class relationships to lean better representations.}\\


\noindent \textbf{R2.3} \textit{Useful intuition to clarify: What does it mean for a target to be uncertain? I found an explanation to this in caption for Figure 3. I suggest you include this earlier in the text to ease understanding.}\\
\indent To clarify the meaning/intuition on the use of the uncertainty, we added a top-level explanation in the introduction section \LU{TODO} and a clarification in the Method section 3.2 as well.
\FG{Refer to 2.2 too?}\\


\noindent \textbf{R2.4} \textit{A non-hyperbolic self-paced learning baseline : From Fig 3 caption ".. Uncertainty indicates the difficulty in classifying specific actions if they are characterized by less or more peculiar..". Is it possible to weigh the usual contrastive learning loss using the distance between positives as a baseline to determine uncertainty?}\\
\indent Thanks for the interesting observation. Generally a measure of uncertainty is highly valued to assess the confidence of the model for a specific prediction. Certainly, using the loss as an index of uncertainty can be effective, however, this metric has more interest at test time when no ground-truth is available. Indeed some effective methods have been introduced \citep{MCDropout}, however the hyperbolic space obtains as a free by-product a measure of uncertainty for each sample (both at train and test time). For SSL, one does not have GT labels even at training time and therefore uses a pretext task and fictitious labels that have no real semantic meaning. Therefore we thing using loss for both training optimization and as an uncertainty measure could lead to overfitting on the pretext task. The borderline case indeed, which is the main problem of in SSL, is when the model collapses to a constant, overfitted and trivial solution. Though further study would be needed to further investigate the answer to you question, and an interesting way might arise from the proposed idea, but we can say that hyperbolic space provides a "loss-independent" uncertainty measure avoiding overfitting in training, e.g., one can have both high and low uncertainty (see Eq. \ref{eq:hyper_distances} for details on hyperbolic distance and uncertainty).
\FG{Some doubts on the match of R question and our answer. He asks to use a baseline to assess uncertainty, and weight contrastive with that. gal and ghahramani use variance of dropout, so it might be applicable to measure the uncertainty during training, although may expensive. Need to object to that or test it.}
\\

\noindent \textbf{R2.5} \textit{Given that your approach is based on a different framework compared to state-of-the-art, you should include results of a non-hyperbolic baseline with BYOL. This will help determine how much of the improvement can be obtained using BYOL based baseline vs MoCo, For example, for Image SSL tasks, BYOL is generally better than MoCo-v2.}\\
\FG{Please note that the required baseline comparison is already contained in Table 3, termed ``w/o hyper''..}
\indent In table 3 we show the result of BYOL baseline without hyperbolic (we named \textit{w/o hyper}). However, thanks to your and \textbf{R3.4}, \textbf{R4.7} comment, we noticed that the result we inserted was a typo and now we corrected it. The top-1 accuracy of the BYOL baseline is 76.9 which is in fact better than the contrastive counterpart SkeletonCLR using MoCo, consistently with the image SSL tasks. The error does not alter the conclusions drawn in the comparison between HYSP and BYOL only, which we reported in the 4.3 section, where we show that by simply introducing hyperbolic self-pacing into BYOL the performance goes up by 5.7\%.
\FG{So, to answer your question, hyperbolic self-pacing improves wrt BYOL by ... \%.}

\PL{Please note that the required baseline comparison is already contained in Table 3, termed ``w/o hyper''. However, thanks to yours and to \textbf{R3.4}, \textbf{R4.7} comments, we noticed a typo in the result and we corrected it. The top-1 accuracy of the BYOL baseline is 76.9 which is in fact better than the contrastive counterpart SkeletonCLR using MoCo, consistently with the image SSL tasks. So, to answer your question, hyperbolic self-pacing improves wrt BYOL by 5.7\%.}
\\


\noindent \textbf{R2.6} \textit{Drop in performance with negatives: While the argument for why negatives cannot be generated in the h space seems convincing, what happens if you generate negatives/apply contrastive learning loss for this experiment on the z space (after projection g) ?}\\
\indent In the transition from Euclidean to hyperbolic for self-supervision methods \FG{remove previous words, not clear that you refer to process of definition of the model, it may be confusing. Rather say: thanks for the observation.}, we tried the suggested experiment. In particular, maintaining the hyperbolic loss between positives $h$ and $\hat{h}$, we tried using a contrastive loss (only for negatives) between $p$ and $\hat{z}$ as for $z$ and $\hat{z}$. In both of these cases, the model doesn't converge or it performs close to the random baseline. Our intuition in this regard is that the model, specifically the encoder $f$, fails to optimize the parameters jointly with respect to two spaces (Euclidean and hyperbolic), given the considerable difference in the concept of distance (linear vs. exponential).
\FG{We should say: we will include or we have included this comment in the paper}

\PL{Thanks for the observation. We tried the suggested experiment and we noticed that by introducing a contrastive loss (using negatives) before the exponential mapping, while keeping the hyperbolic loss after it, the model doesn't converge and performs close to the random baseline. This is probably due to the different optimization needed for the two spaces (euclidean and hyperbolic)}.
\\

\begin{table*}
\caption{Results of transfer learning protocol on PKU-MMD II. We compared directly with the results reported in \citet{thoker2021skeleton}. Here,
After training an encoder with HYSP on the source dataset (NTU-60 and PKU-MMD I), then the pretrained encoder and classifier are jointly fine-tuned on a target dataset (PKU-MMD II) for action classification.}
\centering
\resizebox{0.6\textwidth}{!}{%
\begin{tabular}{l|cc}
\toprule
& \multicolumn{2}{c}{Transfer Learning (PKU-MMD II)}\\
\midrule
Method & \textit{PKU-MMD I} & \textit{NTU-60}\\
\midrule
\LU{NAME} \textit{~\cite{zheng2018unsupervised}} &  43.6 & 44.8 \\
MS$^2$L\textit{~\cite{lin2020ms2l}}  & 44.1 & 45.8 \\
ISC\textit{~\cite{thoker2021skeleton}} & 45.1 & 45.9 \\
\rowcolor[HTML]{ebebeb}
\textbf{HYSP \textit{(ours)}}  & \textbf{50.7} & \textbf{46.3} \\
\bottomrule
\end{tabular}
}
\label{tab:transfer-pkuII}
\end{table*}

\noindent \textbf{R2.7} \textit{Suggestion: I think in addition to linear evaluation, you should evaluate your approach on transfer learning as well. For skeleton-based SSL, NTU $\rightarrow$ PKU I/II is a good option.}\\
\indent Thank you for suggesting this addition. As also recommended in \textbf{R3.3}, we added the transfer learning protocol on PKU-MMD II comparing our results with those of ~\citet{thoker2021skeleton}. Please refer to Table \ref{tab:transfer-pkuII} for the results. Consistently with all other protocols, HYSP succeeds in achieving the state-of-the-art in transfer learning for both NTU-60 to PKU-MMD II and PKU-MMD I to PKU-MMD II. We added the table to the supplementary material (See Appendix D).

\PL{Thank you for suggesting this addition. Please refer to Table \ref{tab:transfer-pkuII} for the results. We also added the table to the supplementary material (See Appendix D).}


\noindent \textbf{R2.8} \textit{The paper includes details on training time. It would be helpful to include details on how much extra compute/traning time is needed due to the use of Riemannian gradient descent.}\\
\indent In \citet{BecGan19} is defined how to implement Riemmanian gradient optimization (c.f. Sec. 2.2). In particular, since a closed form for the gradient is often not defined, the Euclidean gradient $\nabla L(h)$ is calculated and a contraction or conformation is performed at the reference manifold. As also stated in \citet{Guo_2022_CVPR}, a \textit{conformal factor} is multiplied to the Euclidean gradient to obtain the Riemannian $\frac{\partial L}{\partial h}$ gradient. We report the relation in the following equation \ref{eq:riemann_grad}:

\begin{equation}
\begin{split}
    \frac{\partial L_{poin}}{\partial h} & = cf(h) \nabla L_{poin}(h) = \frac{(1 - \|h\|^2)^2}{4} \nabla L_{poin}(h) = \\
    &= \frac{(1-\|h\|^2)^2}{2\sqrt{(1-\|h\|^2)(1-\|\hat{h}\|^2)+\|h-\hat{h}\|^2}} \Biggl(\frac{h-\hat{h}}{\|h-\hat{h}\|} + \frac{h \|h-\hat{h}\|}{1-\|h\|^2}\Biggr),
\end{split}
\label{eq:riemann_grad}
\end{equation}

where $L_{poin}$ is the Poincaré loss and $h$ is the hyperbolic embedding and $cf(h)$ is the conformal factor between Hyperbolic and Euclidean manifold. 
\FG{next sentence is only needed, it seems. One may have everything else is a reference, right?} Adopting only this correction on the gradient, the training time doesn't have any significant variation.

\LU{1.\ Our equation 5 in the paper use nabla symbol for Riemannian gradient while \citet{Guo_2022_CVPR} use nabla for Euclidean one. What to change?}

\LU{2.\ We can discuss however that HNN have a slower training time because of the definition of the "sum" that in the case of Modius addition are really computational expensive w.r.t. Euclidean one. Is this too much to say or not?}
\FG{If you express difference in training time, and it the main reason is not the conformal, then it makes sense to say what makes training time differ mostly.}

\PL{I think this answer it too long. We could just answer the following:}\\
\PL{Adopting RiemanniaSGD instead of SGD does not produce any significant variation in training times since we do not have any hyperbolic layer inside the model.}
\\






\noindent \textbf{Reviewer 3}\\

\noindent \textbf{R3.1} \textit{The proposal seems to be incremental based on prior works. HYSP is not the first method that uses the hyperbolic space in skeleton action recognition \citep{Peng2020MixDI} and uses the BYOL for self-supervised skeleton representation learning \citep{Moliner_2022_CVPR}.}\\
\indent Thank you for bringing these two articles to our attention.  

\noindent We read the first one \citep{Peng2020MixDI} carefully, and we think some really interesting points could be useful for our future works, but actually, we believe also a few significant differences are present with our HYSP. 
\begin{enumerate}
    \item In their work, hyperbolic geometry was mainly introduced because graph data (skeletons) are well-known non-Euclidean structures and then Riemannian space could be a more suitable manifold for the final representation. However, the role of the uncertainty, that we leverage for self-paced SSL, is never mentioned here.

    \item Training is supervised and the latent hierarchy could be derived from the labels. Other works \citep{Chen2020HyperbolicIM, horoPCA, Guo_2022_CVPR} proved that hierarchical labels could be heavily exploited by HNN to achieve much better performance. On the other hand, the use of hyperbolic neural networks without any labels has not been fully explored, analyzing the role of hyperbolic uncertainty in self-supervised training.

    \item The paper aims to design a hyperbolic encoder. In particular, each ST-GCN layer models representation in Poincarè ball to achieve better performance. This point opens an interesting future research path toward a full-hyperbolic model, that is not trivial as we mentioned in our paper (see \textit{hyper. downstream} in the Ablation studies).
\end{enumerate}

\noindent Regarding \citet{Moliner_2022_CVPR}, we have studied their work and the two interesting innovations they introduce (new ad-hoc augmentations and multi-viewpoint sampling). At this time, we tried to reproduce the code on our own as it is not available online, but we could not understand all the details to achieve the same performance. We contacted the authors themselves for clarification on this, but at the moment we have not had a reply to give you a complete explanation in this rebuttal. Then we will try to replicate their implementations in future experiments. However, we still have doubts as to whether this can still be a fair comparison. \PL{Indeed, \citet{Moliner_2022_CVPR} has the following differences when it comes to data processing and augmentation compared to other works:
\begin{itemize}
    \item Skeleton sequences are cropped to 150 frames instead of 50 and, although they provide more information, they also require much more memory for the training.
    \item As input for the model, they concatenate the joint and bone representations along the channel dimension, which can be thought as a 2-stream model. We tried to do the same but we found that the performance actually drop.
    \item They perform what they call Multi-Viewpoint Sampling, which consists in leveraging the viewpoint information provided by the capturing system. Again, we couldn't correctly implement this type of sampling without the code.
\end{itemize}
All the points mentioned above have prevented us from being able to reproduce their results and made us think that their results are not totally comparable with the ones from current state-of-the-art works.
}

Actually, our claim in the third paragraph of the Introduction (Sec.\ 1) is to be the first one to leverage hyperbolic uncertainty to self-pace a self-supervised training. The first insight behind the work stems from the possibility that the self-supervision signal for the pretext task might be enhanced by this additional radius knowledge. Please see also clarification in point \textbf{2.2} for more details.
\\



\noindent \textbf{R3.2} \textit{Why only BYOL?: In my opinion, a better way to show the hyperbolic space is useful is to combine the hyperbolic space with multiple self-supervised learning baselines. From the results in Table 3 (w/ neg.), the hyperbolic space seems not to work well on MoCo.}\\
\indent  As discussed in the previous section, the introduction of hyperbolic space did not stem solely from the need to increase the results of a positive-only Euclidean method, but rather to see whether hyperbolic uncertainty could effectively guide training. As was rightly noted in his commentary and discussed in the related ablation study, the use of negatives is not well defined in a hyperbolic space. Therefore, the introduction of BYOL (like the curriculum learning strategy) was a necessity to test the claim of hyperbolic self-pacing for SSL.

However, several self-supervision frameworks such as SimSiam \citep{Chen2021ExploringSS} have been tried but without additional insights compared to BYOL. 
For future developments, it was planned to use a framework similar to NNCLR \citep{Dwibedi2021WithAL}, which introduces additional positives with hard negative mining (however already introduced in Euclidean space in \citet{guo2022aimclr}). Furthermore, it would be interesting to find a well-posed strategy to introduce contrastive loss with negatives also in the hyperbolic case \LU{we could cite VICReg saying that it is not trivial} as validate HYSP also for the case of SSL image task. However, each baseline framework requires much work to convert the loss, train and fine-tune hyperparameters; therefore we considered it sufficient for our purpose to limit ourselves to the comparison of BYOL and MoCo.\\



\noindent \textbf{R3.3} \textit{The linear evaluation results are not as good as SOTA methods. And the transfer learning results are missing. These two evaluation protocols are more important than the semi-supervised and supervised settings, regarding showing the effectiveness of self-supervised methods, in my opinion.}\\
\indent \textbf{Linear protocol} Following your appropriate \FG{appropriate? maybe remove this attribute} comment and \textbf{R2.1} we \FG{we challenged the submitted results and found that we had neglected the tuning of the batch size hyper-parameter. Adjusting it on the validation set, it yields .. which is line with your observation .. or something on this note} were able to improve our analysis and performance on the linear protocol, obtaining the state-of-the-art on the NTU-60 dataset. As argued in \textbf{R2.1}, compared to the other protocols, the linear one benefits from a significantly smaller batch size. We increased accuracy in the NTU-60 xview from 78.3 to 82.6 (+4.3\%), just reducing the batch size to 32 (as opposed to 512 as it was previously). We report for a full examination  Table \ref{tab:bs_linear}, where we can see the improvement in top-1 accuracy as the batch size changes. Interestingly for NTU-120 we do not have the same increase in accuracy, which remains unchanged, even if we reduce the batch-size value. We added this interesting property also in the supplementary material (see Appendix C) for future follow-ups and, for complete transparency, we will upload checkpoints for all the training.

\textbf{Transfer Learning} Thanks for recommending this improvement. As we also clarified in \textbf{R2.7} we implemented the transfer learning protocol on PKU-MMD II following the setup and results reported in ~\citet{thoker2021skeleton}. Referring to the results in Table \ref{tab:transfer-pkuII} when using NTU-60 and PKU-MMD I as a source dataset, HYSP achieves the state-of-the-art in transferring knowledge to PKU-MMD II. For a complete experimental analysis, we included the table in the supplementary material (see Appendix D).
\\


\noindent \textbf{R3.4} \textit{Table 3: the BYOL-only result (w/o hyper.) may be not reasonable.}\\
\indent Thanks for your observation. Actually, also addressing \textbf{R2.7}, \textbf{R4.7}, we discovered a typo in the result we inserted and have now fixed it (c.f. Table 3 \textit{w/o hyper} for the updated result). Anyway, the error does not change the conclusions in section 4.3 from the comparison between HYSP and BYOL. We demonstrate that performance using the BYOL SSL framework increases in comparison with the MoCo framework, according to the image SSL task. Moreover, the introduction of hyperbolic self-pacing, with HYSP in comparison with BYOL-only, still results effective for better representation (+5.7\%).
\\








\noindent \textbf{Reviewer 4}\\


\noindent \textbf{R4.1} \textit{Parts of the approach do exist in prior works. The authors should further elaborate whether the HYSP is a combination of several methods \citep{grill:hal-02869787, NEURIPS2018_dbab2adc, guo2022aimclr}. However, I think that the paper presents a good study on some of the practices and makes a compelling case for using BYOL for the task.}\\
\indent Thanks for your comment of appreciation. Certainly, our work is based on the aforementioned works. However, as was noted by this comment and \textbf{R4.3}, we do not consider HYSP to be exclusively a combination of various works. In fact, as stated in the third paragraph of the introduction (Sec. 1), our work does not claim to be the first to adopt BYOL in SSL or the use of HNN in the case of skeleton-based action recognition, but rather to use hyperbolic uncertainty as a self-pacing mechanism for SSL for the first time.
To verify this intuition, the use of a positive-only framework such as BYOL (as the curriculum learning strategy) was therefore adopted out of necessity. In fact, the use of contrastive loss with negative samples is ill-posed in hyperbolic space, both from a theoretical point of view and in terms of results (c.f. ablation study \textit{w/ negative}).
\\


\noindent \textbf{R4.2} \textit{HYSP is not the first method to use the positive-only BYOL and the performance of HYSP is not that competitive \citep{Moliner_2022_CVPR}.}\\
\indent 
Thank you for introducing us to the work of \citet{Moliner_2022_CVPR}. As also clarified in the previous point, HYSP does not claim to use BYOL for the first time as an SSL framework for skeleton-based action recognition. In fact, we believe that this intriguing work introduces two interesting novelties (new ad-hoc augmentations and multi-viewpoint sampling) that can be complementary to our work, which instead claims to introduce novel mechanisms for any self-supervision task (as for image task and not only skeleton-based action classification). However, in this period we have tried to replicate the mechanics of the mentioned paper and integrate them into our code, as the code has not been made available by the authors. We have not been able to get the reproduction of the results of the paper for this rebuttal and in this short time we have not received a response from the authors, so we hope to be able to continue this development in the next future.
\\


\noindent \textbf{R4.3} \textit{Although mentioned in the conclusion, I still think that HYSP is more like a general improvement of the self-supervised framework for BYOL combined with hyperbolic space. Measurements on image classification tasks may be more convincing and necessary. I have not seen a unique improvement and analysis for the field of skeleton action recognition.}\\
\indent Thanks for the suggestion; we agree entirely with what you noted. In fact, HYSP is fully implementable with any self-supervision task such as that of images, where we can verify the generality and effectiveness of our proposed method. We have chosen in particular the skeleton-based action recognition task, as it is computationally more accessible to our resources. Moreover going from inputting an image ($256\times256\times3$) to a skeleton ($17\times50\times3$) is computationally much simpler. This allowed us to correctly calibrate the model (loss, hyperparameters, ...) through numerous trainings, with the aim of switching to the images domain once we have acquired this proficiency on a computationally simpler field.
\FG{Here you repeat the statements in conclusions which he knows already. He says "may be more convincing and necessary". We must rebutt this concept. Say that testing on skeleton only is enough, show evidence to convince that the task is enough to state improvement. This is more important than re-stating. They may else reject saying not tested enough.}
\\

\noindent \textbf{R4.4} \textit{Double check the last name and first name of the author of the cited paper, some are confused, such as "Tianyu et al." should be "Guo et al.".}\\
\indent Thank you for the note, we corrected it. 
\\

\noindent \textbf{R4.5} \textit{Please explain Eq.5 in more detail. The conclusion behind Eq.5 cannot be intuitively understood from Eq.5.}\\
\indent In Eq. \ref{eq:riemann_grad} and comment \textbf{R2.8}, we emphasized the conformal factor $cf(h)$ that explicit the difference between Euclidean gradient $\nabla L_{Poin}$ and the Riemannian one $\frac{\partial L}{\partial h}$. As stated in Section 3.2.1, depending on the phase of the training, and specifically the values of $\|h\|, \|\hat{h}\|$ and $\|h - \hat{h}\|$, the gradient affect the learning in a specific way. Indeed also with the help of Figure 2, we can differentiate three main phases:

\begin{itemize}
    \item \textbf{Phase 1}: After the random initialization of the parameters, the network represents all the embedding on the edge of the Poincaré ball. This means that both $\|h\| \approx 1$ and $\|\hat{h}\| \approx 1$. However, the representations of $h$ and $\hat{h}$ are still random as the learning process did not take place and this means that the quantity $\| h - \hat{h} \|$ is positive and relatively far from being zero. However, this distance will be minimized during training because by minimizing the Poincaré distance we automatically decrease the Euclidean $L_2$ distance. Then under the condition of $1 - \|h\|^2 \approx 0$, $1 - \|\hat{h}\|^2 \approx 0$ and $\|h - \hat{h}\| > 0$ it results in:
    \begin{equation}
        \frac{(1-\|h\|^2)^2}{2\sqrt{(1-\|h\|^2)(1-\|\hat{h}\|^2)+\|h-\hat{h}\|^2}} \Biggl(\frac{h-\hat{h}}{\|h-\hat{h}\|} + \frac{h \|h-\hat{h}\|}{1-\|h\|^2}\Biggr) \approx 0,
    \end{equation}
    
    As also studied in the work \citet{Guo_2022_CVPR}, this is due to the conformal factor which dominates all the other terms in the gradient. Because of this Hyperbolic NN suffers from vanishing gradient at the early stages of training. To address this problem clipping features technique is proposed \citep{Guo_2022_CVPR} avoiding initialization on the edge of the Poincaré ball. However, we tackled the problem from a different perspective. Indeed while Euclidean loss minimizes the angle distance between the embeddings $h$ and $\hat{h}$, the hyperbolic loss minimizes angle and radius (certainty) jointly. The latter causes the problem of vanishing gradient so we removed its contribution and, leveraging the conformal property of the angle between Euclidean and Hyperbolic space, we adopt cosine loss in the first stages of the training (c.f. Sec 3.2.3 for more details).

    \item \textbf{Phase 2}: Once the training starts, the representation of $h$ is optimized to match $\hat{h}$ minimizing the Poincarè distance between them. This means $h$ departs from the edge of the ball ($1 - \|h\|^2 > 0$) moving along the geodesic towards $\hat{h}$. In this phase then $\|h - \hat{h}\|$ starts to reduce faster because we are optimizing both angle and radius of each representation, but until the two representations are not meaningful we still have $\|h - \hat{h}\|> 0$. The key point insight behind Eq. 5 of the paper relies on this phase. In fact, the gradient is weighted differently for each term by the term $1 - \|\hat{h}\|^2$ in the denominator. The target embeddings that are more certain $1 - \|\hat{h}\|^2 \approx 0$ drive the training because they weights the gradient more, while the ones that are less certain $1 - \|\hat{h}\|^2 > 0$ are also less important for the optimization because the relative gradient is lower. We can summarize this observation with the following property:
    
    \begin{equation} 
        \|\hat{h}_1\| > \|\hat{h}_2\| \implies \frac{\partial L_{poin}(h_1, \hat{h}_1)}{\partial h_1} > \frac{\partial L_{poin}(h_2, \hat{h}_2)}{\partial h_2}
    \end{equation}

    \item \textbf{Phase 3}: In this final step we have a degradation of the performance because each representation collapse to the origin of the ball. This happens because the hyperbolic distance between two points in the Poincaré ball varies exponentially if we move toward the edge of the ball. Then the following property holds:

    \begin{equation}
        \begin{split}
        \|h_1-\hat{h}_1\| &= \|h_2-\hat{h}_2\| \\
        \|h_1\| &\geq \|h_2\|  \qquad \implies L_{Poin}(h_1, \hat{h}_1) \geq L_{Poin}(h_2, \hat{h}_2), \\
        \|\hat{h}_1\| &\geq \|\hat{h}_2\|
        \end{split}
        \label{eq:hyper_distances}
    \end{equation}

    Please note that in Euclidean space the distances don't change with respect relative position of the points with the origin, in fact, under the same condition it holds $d_{Euc}(h_1, \hat{h}_1) = d_{Euc}(h_2, \hat{h}_2)$. Due to this particular property of hyperbolic space, from a specific moment that we will discuss now, the model reduces the distances between $h$ and $\hat{h}$ shifting them towards the origin where the distances are reduced. This begins to have a negative impact on training as $\hat{h}$ also begins to move from the edge. The target encoder $\hat{f}$ in fact is updated with the momentum and this causes $\hat{h}$ to be updated slower than $h$. Thus the negative influence emerging from the property in Eq. \ref{eq:hyper_distances} has a delayed effect, leaving the model the ability to learn meaningful representations.
    
\end{itemize}

\noindent We updated the supplementary material (see Appendix E) with all these detailed insights behind Eq.\ 5 to help readers understand the meaning of hyperbolic self-pacing.


\noindent \textbf{R4.6} \textit{In Table 1, SkeletonCLR also uses negative samples.}\\
\indent Thanks for the remark; we added the missing checkmark. 
\\

\noindent \textbf{R4.7} \textit{Does "w/o hyper." in Table 3 mean using BYOL directly? If yes, I think the accuracy is unsatisfactory (see weekness2). If not, please explain in more detail and give the result of using BYOL directly.}\\
\indent Thanks for your remark, also addressing \textbf{R3.4}, we find that the number we reported is not correct and we fixed it in Table 3. In any case, the result of the comparison between HYSP and BYOL in section 4.3 remains unaffected by the error. In comparison to the MoCo (w/ neg) SSL framework, our HYSP performs better, as expected also from the results of BYOL vs.\ MoCo in the image SSL tasks. Indeed, hyperbolic self-pacing was still effective for better representation (+5.7\% top-1 accuracy) when HYSP was used instead of BYOL-only.
\\







\noindent In view of all the fruitful comments, we believe we have improved the analysis proposed and addressed all of the raised concerns. \\Please let us know if any further improvement is needed.\\



\noindent Sincerely,\\
Authors
